Optimal Sequence-Based LQG Control over TCP-like Networks Subject to Random Transmission Delays and Packet Losses

This paper addresses the problem of sequence-based controller design for Networked Control Systems (NCS), where control inputs and measurements are transmitted over TCP-like network connections that are subject to stochastic packet losses and time-varying packet delays. At every time step, the controller sends a sequence of predicted control inputs to the actuator in addition to the current control input. In this sequence-based setup, we derive an optimal solution to the Linear Quadratic Gaussian (LQG) control problem and prove that the separation principle holds. Simulations demonstrate the improved performance of this optimal controller compared to other sequence-based approaches.

==> 40_stability.tex <==
%%%%%%%%%%%%%%%%%% Invertability %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
	&= \min_{\vec{U}_{N-2}} \left[ \E \left\{ \rvec{\xi}_{N-2}\tr \tilde{\mat{Q}}_{N-2} \rvec{\xi}_{N-2} + \vec{U}_{N-2}\tr \tilde{\mat{R}}_{N-2} \vec{U}_{N-2}  \right. \right. \\ 
	 & + \rvec{\xi}_{N-1}\tr \tilde{\mat{K}}_{N-1} \rvec{\xi}_{N-1} + \E \left\{ \tilde{\rvec{w}}_{N-1}\tr \mat{K}_{\theta_{N}} \tilde{\rvec{w}}_{N-1} | \mathcal{I}_{N-1} \right\} \left. \left. | \mathcal{I}_{N-2} \right\} \right] \\
%
  &= \rvec{\xi}_{N-2}\tr \E \left\{ \tilde{\mat{Q}}_{N-2} + \tilde{\mat{A}}_{N-2}\tr \tilde{\mat{K}}_{N-1} \tilde{\mat{A}}_{N-2} | \mathcal{I}_{N-2} \right\} \rvec{\xi}_{N-2} \\
   & + \E \left\{ \tilde{\rvec{w}}_{N-1}\tr \mat{K}_{\theta_{N}} \tilde{\rvec{w}}_{N-1} | \mathcal{I}_{N-2} \right\} + \E \left\{ \tilde{\rvec{w}}_{N-2}\tr \tilde{\mat{K}}_{N-1} \tilde{\rvec{w}}_{N-2} | \mathcal{I}_{N-2} \right\} \\
   & + \min_{\vec{U}_{N-2}} \left[ \vec{U}_{N-2}\tr \E \left\{  \tilde{\mat{R}}_{N-2} + \tilde{\mat{B}}_{N-2}\tr \tilde{\mat{K}}_{N-1} \tilde{\mat{B}}_{N-2} | \mathcal{I}_{N-2} \right\}  \vec{U}_{N-2} 
   \right] \\
   & + 2 \cdot \rvec{\xi}_{N-2}\tr \E \left\{ \tilde{\mat{A}}_{N-2}\tr \tilde{\mat{K}}_{N-1} \tilde{\mat{B}}_{N-2} | \mathcal{I}_{N-2} \right\}  \vec{U}_{N-2} \\

Due to \ref

\begin{eqnarray}
	&&\tilde{\mat{R}}_k + \tilde{\mat{B}}_k\tr \mat{K}_k \tilde{\mat{B}}_k \\
	&&= \mat{J}_k\tr \mat{R}_k \mat{J}_k + \begin{bmatrix} \mat{J}_k\tr \cdot {\mat{B}}_k\tr & \mat{G}\tr \end{bmatrix} \mat{K}_k \begin{bmatrix} \mat{B}_k \cdot {\mat{J}}_k \\ \mat{G} \end{bmatrix}\\
%
	&&=\begin{bmatrix} \sigma_0^2\mat{R}_k &\mat{0} \\ \mat{0} & \mat{0} \end{bmatrix} \\ 
	&& + \begin{bmatrix}  \sigma_0 \mat{B}_k\tr & \mat{0} & \mat{0} \\ \mat{0} &\mat{I} &  \mat{0}  \end{bmatrix} \begin{bmatrix}\mat{K}_{11} & \mat{K}_{12} & \mat{K}_{13} \\ \mat{K}_{21} & \mat{K}_{22} & \mat{K}_{23} \\ \mat{K}_{31} & \mat{K}_{32} & \mat{K}_{33}\end{bmatrix} 
		 \begin{bmatrix}  \sigma_0 \mat{B}_k & \mat{0}  \\ \mat{0} &\mat{I} \\ \mat{0} & \mat{0} \end{bmatrix} \nonumber\\
%
	&&=\begin{bmatrix} \sigma_0^2\mat{R}_k &\mat{0} \\ \mat{0} & \mat{0} \end{bmatrix} + 
	\begin{bmatrix}  \sigma_0 \mat{B}_k\tr & \mat{0} & \mat{0} \\ \mat{0} &\mat{I} &  \mat{0}  \end{bmatrix}
	\begin{bmatrix}  \sigma_0 \mat{K}_{11} \mat{B}_k & \mat{K}_{12}\\ \sigma_0 \mat{K}_{21} \mat{B}_k & \mat{K}_{22} \\
	\sigma_0 \mat{K}_{31} \mat{B}_k & \mat{K}_{32} \end{bmatrix} \nonumber \\
%
	&&=\begin{bmatrix} \sigma_0^2\mat{R}_k &\mat{0} \\ \mat{0} & \mat{0} \end{bmatrix} + 
	\begin{bmatrix}  \sigma_0^2 \mat{B}_k\tr \mat{K}_{11}\mat{B}_k & \sigma_0 \mat{B}_k \mat{K}_{12} \\ \sigma_0 \mat{K}_{21} \mat{B}_k & \mat{K}_{22} \end{bmatrix}\\
%
	&&= \begin{bmatrix}  \sigma_0^2 \left(\mat{R}_k + \mat{B}\tr_k \mat{K}_{11}\mat{B}_k\right) & \sigma_0 \mat{B}\tr_k \mat{K}_{12} \\ \sigma_0 \mat{K}_{21} \mat{B}_k & \mat{K}_{22} \end{bmatrix}
\end{eqnarray}

\begin{eqnarray}
&&\tilde{\mat{A}}_k\tr \mat{K} \tilde\mat{B}_k \\
&&= \begin{bmatrix} \mat{A}_k\tr & \mat{0} & \mat{0}\\ \mat{H}_k\tr \cdot \mat{B}_k\tr & \mat{0} &\bar{\mat{F}}\tr \end{bmatrix}
\begin{bmatrix}\mat{K}_{11} & \mat{K}_{12} & \mat{K}_{13} \\ \mat{K}_{21} & \mat{K}_{22} & \mat{K}_{23} \\ \mat{K}_{31} & \mat{K}_{32} & \mat{K}_{33}\end{bmatrix} 
	 \begin{bmatrix}  \sigma_0 \mat{B}_k & \mat{0}  \\ \mat{0} &\mat{I} \\ \mat{0} & \mat{0} \end{bmatrix} \nonumber\\
%
&&= \begin{bmatrix} \mat{A}_k\tr & \mat{0} & \mat{0}\\ \mat{H}_k\tr \cdot \mat{B}_k\tr & \mat{0} &\bar{\mat{F}}\tr \end{bmatrix}
	\begin{bmatrix}  \sigma_0 \mat{K}_{11} \mat{B}_k & \mat{K}_{12}\\ \sigma_0 \mat{K}_{21} \mat{B}_k & \mat{K}_{22} \\
	\sigma_0 \mat{K}_{31} \mat{B}_k & \mat{K}_{32} \end{bmatrix} \nonumber \\
%
&&= \begin{bmatrix}  \sigma_0 \mat{A}_k\tr \mat{K}_{11} \mat{B}_k &  \mat{A}_k\tr \mat{K}_{12}\\ \sigma_0 \mat{H}_k\tr  \mat{B}_k\tr  \mat{K}_{11} \mat{B}_k + \bar{\mat{F}}\tr \mat{K}_{31} \mat{B}_k & \sigma_0 \mat{H}_k\tr  \mat{B}_k\tr  \mat{K}_{12} + \bar{\mat{F}}\tr \mat{K}_{32}\end{bmatrix} \\
%
&&= \begin{bmatrix}  \sigma_0 \mat{A}_k\tr \mat{K}_{11} \mat{B}_k &  \mat{A}_k\tr \mat{K}_{12}\\ \bar{\mat{F}}\tr \mat{K}_{31} \mat{B}_k & \bar{\mat{F}}\tr \mat{K}_{32}\end{bmatrix}
\end{eqnarray}

\begin{eqnarray}
\begin{bmatrix}  \sigma_0 \mat{A}_k\tr \mat{K}_{11} \mat{B}_k \sigma_0^2 \left(\mat{R}_k + \mat{B}\tr_k \mat{K}_{11}\mat{B}_k\right) \sigma_0 \mat{B}_k\tr \mat{K}_{11} \mat{A}_k & \sigma_0 \mat{A}_k\tr \mat{K}_{11} \mat{B}_k \sigma_0^2 \left(\mat{R}_k + \mat{B}\tr_k \mat{K}_{11}\mat{B}_k\right) \sigma_0  \mat{B}_k\tr  \mat{K}_{11} \mat{B}_k \mat{H}_k \\ 
 \sigma_0 \mat{H}_k\tr  \mat{B}_k\tr  \mat{K}_{11} \mat{B}_k  \sigma_0^2 \left(\mat{R}_k + \mat{B}\tr_k \mat{K}_{11}\mat{B}_k\right) \sigma_0 \mat{B}_k\tr \mat{K}_{11} \mat{A}_k &
\sigma_0 \mat{H}_k\tr  \mat{B}_k\tr  \mat{K}_{11} \mat{B}_k  \sigma_0^2 \left(\mat{R}_k + \mat{B}\tr_k \mat{K}_{11}\mat{B}_k\right) \sigma_0  \mat{B}_k\tr  \mat{K}_{11} \mat{B}_k \mat{H}_k \\ 
 \end{bmatrix}
\end{eqnarray}
\newpage
\begin{eqnarray}
&&K_2 = \begin{bmatrix}
	\mat{Q}_k & \mat{0} \\
	\mat{0}   & \mat{H}_{k}\tr \mat{R}_k \mat{H}_{k}
	\end{bmatrix}
	+ \begin{bmatrix} \mat{A}_k\tr \mat{K}_{11} \mat{A}_k & \mat{A} \mat{K}_{11} \mat{B}_k \mat{H}_k \\
										\mat{H}_k\tr \mat{B}_k\tr \mat{K}_{11} \mat{A} & \mat{H}_k\tr \mat{B}_k\tr\mat{K}_{11} \mat{B}_k \mat{H}_k 
	\end{bmatrix}
\end{eqnarray}

To analyze the stability of the closed-loop system, we study the expected average cost per stage if the terminal time emerges infinity. \com{why?, mean square stability} 
\begin{align}. 
	J^{*}_0(\infty) & = \displaystyle\lim_{k\rightarrow\infty} \frac{1}{k} J^{*}_0(k) \nonumber \\
									& = \displaystyle\lim_{k\rightarrow\infty} \frac{1}{k} 
									\E \left\{ \rvec{\xi}_{k}\tr {\mat{K}}_{k+1} \rvec{\xi}_{k} | \mathcal{I}_{k} \right\}  \label{eq:Jkinfty}\\
							& + \displaystyle\sum_{i=k}^{K-1}\E \left\{ \tilde{\rvec{w}}_{i}\tr \mat{K}_{i+1} \tilde{\rvec{w}}_{i} | \mathcal{I}_{i} \right\}  \nonumber \\
	& + \displaystyle\sum_{i=k}^{K-1}\E \left\{ \left( \rvec{\xi}_{i+1}\tr - \E \left\{ \rvec{\xi}_{i+1}\tr | \mathcal{I}_{i+1}\right\} \right) \mat{P}_{i+1} \right. \nonumber \\
  & \hspace{0.35cm} \times \left. \left( \rvec{\xi}_{i+1} - \E \left\{ \rvec{\xi}_{i+1} | \mathcal{I}_{i+1}\right\}\right)| \mathcal{I}_{i} \right\} \nonumber \ .
\end{align}
If $J^{*}_0(\infty)$ is bounded, then the closed-loop system is stable. The average cost given by ... are unbounded iff one or more of the summands are unbounded since all summands are positive. In the following subsections we examine the summands separately:

\subsection{Cost dependend on control}
\begin{equation}
	\displaystyle\lim_{k\rightarrow\infty} \frac{1}{k} 
									\E \left\{ \rvec{\xi}_{k}\tr {\mat{K}}_{k+1} \rvec{\xi}_{k} | \mathcal{I}_{k} \right\}  \\
\end{equation}
Derivation of an upper bound of
\begin{align}
  \E &\left\{ \mat{K}_k | \theta_{k-1} = j \right\} \nonumber \\ 
  					& = \left[ \displaystyle\sum_{i=0}^{N+1} q_{ji} \left(\tilde{\mat{Q}}_{|i}+ \left(\tilde{\mat{A}}_{|i}\right)\tr \E \left\{ \mat{K}_{k+1}| \theta_k = i \right\}\tilde{\mat{A}}_{|i}\right) \right] \nonumber \\
						& - \left[\displaystyle\sum_{i=0}^{N+1} q_{ji}  \left(\tilde{\mat{A}}_{|i}\right)\tr \E \left\{ {\mat{K}}_{k+1} | \theta_k = i \right\} \tilde{\mat{B}}_{|i}\right] \nonumber \\
						& \times \left[ \displaystyle\sum_{i=0}^{N+1} q_{ji}  \left( \tilde{\mat{R}}_{|i} + \left(\tilde{\mat{B}}_{|i}\right)\tr \E \left\{ {\mat{K}}_{k+1} | \theta_k = i \right\} \tilde{\mat{B}}_{|i}  \right) \right]^\dagger \nonumber \\
						& \times \left[ \displaystyle\sum_{i=0}^{N+1} q_{ji}  \left(\tilde{\mat{B}}_{|i}\right)\tr \E \left\{ {\mat{K}}_{k+1} | \theta_k = i \right\} \tilde{\mat{A}}_{|i} \right] \ , \label{eq:KkSum}
\end{align}
defining the matrix
\begin{align}
	&\mat{M}_{k|i, j} = \\
	&\begin{bmatrix} 
%						q_{ji}^3\left(\tilde{\mat{Q}}_{|i}+ \tilde{\mat{A}}_{|i}\tr \mat{K}_{k+1|i}\tilde{\mat{A}}_{|i}\right) 
%						& q_{ji}\left(\tilde{\mat{A}}_{|i}\tr \mat{K}_{k+1|i} \tilde{\mat{B}}_{|i}\right) \\
%						q_{ji}\left(\tilde{\mat{B}}_{|i}\tr \mat{K}_{k+1|i} \tilde{\mat{A}}_{|i}\right)
%						& q_{ji}\left(\tilde{\mat{R}}_{|i} + \tilde{\mat{B}}_{|i}\tr \mat{K}_{k+1|i}\tilde{\mat{B}}_{|i}\right)
						q_{ji}^3 \mat{V}\mat{T}^\dagger\mat{V}\tr  &  q_{ji}\mat{V} \\
						q_{ji}\mat{V}\tr
						& q_{ji}\mat{T}
	\end{bmatrix} \\
\end{align}
Schur theorem: $\mat{M} \geq 0$ since $\mat{C} \geq 0, \left(\mat{I} - \mat{A}\mat{A}^\dagger\right) \mat{B} = 0, \mat{A}- \mat{B}\mat{C}^\dagger\mat{B}\tr \geq 0$
\com{AAdagger B = 0?}
Since $\mat{M} \geq 0$ it holds that
\begin{align}
	&\displaystyle\sum_{i=0}^{N+1} \mat{M}_{k|\theta_k = i, j} \geq 0
\end{align}
Therefore lower bound:
\begin{align}
	\begin{bmatrix}
		&\displaystyle\sum_{i=0}^{N+1} q_{ji}^3 \mat{V}\mat{T}^\dagger\mat{V}\tr  
		&\displaystyle\sum_{i=0}^{N+1}q_{ji}\mat{V} \\
		&\displaystyle\sum_{i=0}^{N+1} q_{ji}\mat{V}\tr
		&\displaystyle\sum_{i=0}^{N+1}q_{ji}\mat{T}
	\end{bmatrix} \geq 0
\end{align}
\begin{align}
	& \left(\displaystyle\sum_{i=0}^{N+1} q_{ji}^3 \mat{V}\mat{T}^\dagger\mat{V}\tr \right) \\ 
	& \geq \left(\displaystyle\sum_{i=0}^{N+1}q_{ji}\mat{V}\right)
	\left(\displaystyle\sum_{i=0}^{N+1}q_{ji}\mat{T}\right)^\dagger  \left(\displaystyle\sum_{i=0}^{N+1} q_{ji}\mat{V}\tr\right)
\end{align}

Upper bound:
\begin{align}
	\begin{bmatrix}
		&\displaystyle\sum_{i=0}^{N+1} q_{ji}\left(2\cdot\mat{S}-\mat{V}\mat{T}^\dagger\mat{V}\tr  \right)
		&\displaystyle\sum_{i=0}^{N+1}q_{ji}\mat{V} \\
		&\displaystyle\sum_{i=0}^{N+1} q_{ji}\mat{V}\tr
		&\displaystyle\sum_{i=0}^{N+1}q_{ji}\mat{T}
	\end{bmatrix} \geq 0
\end{align}

\subsection{Cost dependend on state estimation}
It holds for the last summand $e_{i+1|i+1} = \left( \rvec{\xi}_{i+1} - \E \left\{ \rvec{\xi}_{i+1} | \mathcal{I}_{i+1}\right\} \right)$
\begin{align}
  & \displaystyle\sum_{i=k}^{K-1}\E \left\{ \rvec{e}_{i+1|i+1}\tr \mat{P}_{i+1} \rvec{e}_{i+1|i+1} | \mathcal{I}_{i} \right\} \no  \\
  = & {\rm Tr} \E \mat{P}_{i+1} \rvec{e}_{i+1|i+1} \rvec{e}_{i+1|i+1}\tr \no
\end{align}



%In this section we will derive a criterion for closed-loop stability of the proposed controller. %We concentrate on the case where the weighting factors of the virtual control inputs are approximated by its steady state distribution described by Eq. (\ref{eq:alphaInfty}). 
%%\begin{remark}
%%It should be noted, that, although an approximation is used in the controller design, the derived stability results for this controller are exact and not approximated.
%%\end{remark}
%To that end, first, a model of network and actuator is derived, that, in a second step, will be combined with the model of the plant (\ref{eq:system}) and the controller (\ref{eq:LSchlange}).
%%
%% --------------------------- sub:Combined model -------------------------
%\subsection{Combined Model of Network and Actuator}
%Based on $\vec{\eta}_k$ and $\rv{\theta}_k$ as defined in section \ref{sub:VCI}, the combined state space model of network and actuator can be formulated similar as in \cite{Xiao00} as
%%
%\begin{eqnarray}
%	\vec{\eta}_{k+1} & = & \mat{F} \vec{\eta}_k + \mat{G} U_k \label{eq:netwAndAct1} \ , \\
%  \hat{\vec{u}}_k  & = & \mat{H}_{\theta_k} \vec{\eta}_k + \mat{J}_{\theta_k} U_k \label{eq:netwAndAct2} \ ,
%\end{eqnarray}
%%%
%%with
%%%
%%\begin{align*}
%%	\mat{F} &= 
%%	\begin{bmatrix}
%%		\mat{0}_{nN\times n} & \mat{0}_{nN \times n(N-1)} & \mat{0}_{nN\times n} & \mat{0}_{nN\times n(N-2)} &\cdots & \mat{0}_{nN\times n} & \mat{0}_{nN\times n} & \mat{0}_n\\
%%			\mat{0}_{n(N-1)\times n} & \mat{I}_{n(N-1)} & \mat{0}_{n(N-1)\times n} & \mat{0}_{n(N-1)\times n(N-2)} &\cdots & \mat{0}_{n(N-1)\times n} & \mat{0}_{n(N-1)\times n} & \mat{0}_n\\
%%		\mat{0}_{n(N-2) \times n} & \mat{0}_{n(N-2) \times n(N-1)} & \mat{0}_{n(N-2)\times n} & \mat{I}_{n(N-2)} &\cdots & \mat{0}_{n(N-2) \times n} & \mat{0}_{n(N-2) \times n} & \mat{0}_n\\
%%		\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots & \vdots\\
%%		\mat{0}_n & \mat{0}_{n \times n(N-1)} & \mat{0}_n & \mat{0}_{n \times n(N-2)} &\cdots & \mat{I}_n & \mat{0}_n & \mat{0}_n \\
%%		\mat{0}_n & \mat{0}_n & \mat{0}_n & \mat{0}_n & \cdots & \mat{0}_n & \mat{0}_n & \mat{I}_n \\
%%	\end{bmatrix} \\ \nonumber \  \\
%%
%%\end{align*}
%%	\mat{G} &= 
%%	\begin{bmatrix}
%%		\mat{0}_{nN \times n} & \mat{I}_{nN}\\
%%		\mat{0}_{n(N-1) \times n}  & \mat{0}_{n(N-1) \times nN}\\
%%		\vdots & \vdots\\
%%		\mat{0}_n & \mat{0}_{n \times nN}
%%	\end{bmatrix} \ , \ \ \ \ \ \ 
%%	%
%%  \mat{J}_{\theta_k} =
%%	\begin{bmatrix}
%%	  \delta_{(\theta_k, 0)}\mat{I}_n & \mat{0}_{n \times nN}
%%	\end{bmatrix} \ , \ \ \ \ \ \ \ 
%%%
%%	\mat{H}_{\theta_k} =	
%%	\begin{bmatrix}
%%		\delta_{(\theta_k, 1)}\mat{I}_n \\ 
%%		\mat{0}_{n\times n(N-1)} \\  
%%		\delta_{(\theta_k, 2)}\mat{I}_n \\
%%		\mat{0}_{n\times n(N-2)} \\
%%		\vdots \\
%%		\delta_{(\theta_k, N)}\mat{I}_n  \\
%%		\delta_{(\theta_k, N+1)}\mat{I}_n  
%%		\end{bmatrix}^T ,
%%\end{align*}
%%%
%%where $\delta_{(\theta_k, i)}$ is the Kronecker delta function defined as
%%%
%%\begin{eqnarray*}
%%	\delta_{(\theta_k, i)} = 
%%	\left\{ \begin{array}{rcl}
%%		1 & \mbox{if} & \theta_k = i\\
%%		0 & \mbox{if} & \theta_k \neq i
%%	\end{array}\right. \ .
%%\end{eqnarray*}
%%
%with\\
%\begin{equation*}
%	\begin{aligned}
%%
%		\mat{F} &= 
%		\begin{bmatrix}
%			\mat{0} & \mat{0} & \mat{0} & \mat{0} &\cdots & \mat{0} & \mat{0}\\
%			\mat{0} & \mat{I} & \mat{0} & \mat{0} &\cdots & \mat{0} & \mat{0}\\
%			\mat{0} & \mat{0} & \mat{0} & \mat{I} &\cdots & \mat{0} & \mat{0}\\
%			\vdots & \vdots & \vdots & \vdots & \ddots & \vdots & \vdots \\
%			\mat{0} & \mat{0} & \mat{0} & \mat{0} &\cdots & \mat{I} & \mat{0} \\
%		\end{bmatrix}  \nonumber ,
%	\end{aligned}
%%
%	\begin{aligned}
%		\mat{G} = &
%		\begin{bmatrix}
%			\mat{0} & \mat{I}\\
%			\mat{0} & \mat{0}\\
%		\end{bmatrix} , \\ \\
%	%
%	  \mat{J}_{\theta_k} = &
%		\begin{bmatrix}
%  		\delta_{(\theta_k,0)}\,\mat{I} & \mat{0}
%		\end{bmatrix} ,
%	\end{aligned}
%\end{equation*}
%\begin{equation}
%\begin{aligned}
% \mat{H}_{\theta_k} &=	
%  	\begin{bmatrix}
%  		\delta_{(\theta_k,1)}\,\mat{I} &
%  		\mat{0}&  
%			\delta_{(\theta_k,2)}\,\mat{I} &
%			\mat{0}&
%			\cdots &
%			\delta_{(\theta_k,N)}\,\mat{I}
%  	\end{bmatrix} \ ,  \nonumber
%\end{aligned}
%\end{equation}
%where the \mat{0}'s are matrices with all elements equal to zero and the \mat{I}'s are identity matrices, each of appropriate dimension. The term $\delta_{(\theta_k, i)}$ is the Kronecker delta, which is defined as
%\begin{eqnarray*}
%	\delta_{(\theta_k, i)} = 
%	\left\{ \begin{array}{rcl}
%		1 & \mbox{if} & \theta_k = i\\
%		0 & \mbox{if} & \theta_k \neq i
%	\end{array}\right. \ .
%\end{eqnarray*}
%%
%% --------------------------------------- sub: CL-Model ---------------------
%\subsection{Model of the Closed-Loop System}
%By using the augmented state $\rvec{\psi}_k$ from (\ref{eq:psi}) and combining (\ref{eq:system}), (\ref{eq:netwAndAct1}), and (\ref{eq:netwAndAct2}), it holds
%%
%\begin{align*}
%\rvec{\psi}_{k+1} & = 
%	\begin{bmatrix}
%		\mat{A} & \mat{B} \cdot \mat{H}_{\theta_k}\\
%		\mat{0}  & \mat{F}
%	\end{bmatrix}
%	\rvec{\psi}_k +
%	\begin{bmatrix}
%		\mat{B} \cdot \mat{J}_{\theta_k}\\
%		\mat{G}
%	\end{bmatrix}
%	U_k + 
%	\begin{bmatrix}
%		\rvec{w}_k \\
%		\mat{0}
%	\end{bmatrix} \ . 
%	%
%\end{align*}
%%
%Using (\ref{eq:LSchlange}) results in
%%
%\begin{align}
%	\rvec{\psi}_{k+1} & = \left[
%	\begin{bmatrix}
%		\mat{A} & \mat{B} \cdot \mat{H}_{\theta_k}\\
%		\mat{0} & \mat{F}
%	\end{bmatrix}
%	- 
%	\begin{bmatrix}
%		\mat{B} \cdot \mat{J}_{\theta_k} \cdot \tilde{\mat{L}}\\
%		\mat{G} \cdot \tilde{\mat{L}}
%	\end{bmatrix}
%	 \right] \rvec{\psi}_k + 
%	\begin{bmatrix}
%		\rvec{w}_k \\
%		\mat{0}
%	\end{bmatrix} \nonumber \\
%	%
%	& = \tilde\mat{A}_{\theta_k} \rvec{\psi}_k + \tilde{\rvec{w}}_k  \ . \label{eq:closedLoopedSystem}
%\end{align}
%%
%The closed-loop system described by (\ref{eq:closedLoopedSystem}) can be interpreted as an inhomogeneous Markovian jump linear system (MJLS). 
%For this kind of system, several results on mean square stability are available in the literature, e.g.,  \cite{Costa05} and \cite{Feng92}. 
%In the following, we adopt the concept of mean square stability and proof from \cite{Costa05}.
%%----------------- MSS definition -----------------------------
%\begin{definition}
%	The system (\ref{eq:closedLoopedSystem}) with Markovian jump parameter $\theta_k$ is mean square stable (MSS), if for any initial condition $\theta_0 \in \left\{0, 1, \cdots, N\right\}$ and $\rvec{\psi}_0 \in \mathbb{R}^{d+s}$ there exist a bounded $\vec{\mu} \in \mathbb{R}^{d+s}$ and a symmetric positive-semidefinite matrix $\mat{M}$ (independent of $\rvec{\psi}_0$ and $\theta_0$) such that
%	\begin{eqnarray}
%		\lim\limits_{k\rightarrow \infty} E\left\{ \rvec{\psi}_k \right\} = \vec{\mu}\ , \\
%		\lim\limits_{k\rightarrow \infty} E\left\{ \rvec{\psi}_k \rvec{\psi}_k^T\right\} = \mat{M} \ .
%	\end{eqnarray}
%\end{definition}
%%---------------------- Stability theorem -----------------------------
%\begin{theorem} 
%		The system (\ref{eq:closedLoopedSystem}) with Markovian jump parameter $\theta_k$ and transition matrix $\mat{P}$ is stable in the mean square sense, if and only if 
%	\begin{eqnarray}
%		r_\sigma((\mat{P}^T \otimes \mat{I}_{n^2})\cdot {\rm diag}[\tilde{\mat{A}}_i \otimes \tilde{\mat{A}}_i]) < 1 \ ,
%	\end{eqnarray}
%	where $r_\sigma\(\mat{M}\)$ is the spectral radius of $\mat{M}$ and ${\rm diag}\left[ \mat{S}_i\right]$ is the block diagonal matrix built by $\mat{S}_i$ in the diagonal with $i = \{0, 1, ..., N\}$ and zero everywhere else, i.e.,
%	\begin{equation}
%	{\rm diag}\left[\mat{S}_i\right] =
%		\begin{bmatrix}
%			\mat{S}_0 & \mat{0} & \cdots & \mat{0}\\
%			\mat{0} & \mat{S}_1 & \cdots & \mat{0}\\
%			\vdots & \vdots & \vdots & \vdots\\
%			\mat{0} & \mat{0} & \cdots & \mat{S}_N
%		\end{bmatrix} \ .
%	\end{equation}
%\end{theorem}
%\begin{proof}
%The result follows from theorem 3.9 and 3.33 in \cite{Costa05}.
%\end{proof}
